Interaction Order Prediction for Temporal Graphs

Link prediction in graphs is a task that has been widely investigated. It has been applied in various domains such as knowledge graph completion, content/item recommendation, social network recommendations and so on. The initial focus of most research was on link prediction in static graphs. However, there has recently been abundant work on modeling temporal graphs, and consequently one of the tasks that has been researched is link prediction in temporal graphs. However, most of the existing work does not focus on the order of link formation, and only predicts the existence of links. In this study, we aim to predict the order of node interactions.

==> extra.tex <==
Graph2Seq: https://arxiv.org/abs/1804.00823
GitHub: https://github.com/IBM/Graph2Seq

https://github.com/Cartus/DCGCN

https://paperswithcode.com/task/graph-to-sequence

https://aclanthology.org/2020.acl-main.640.pdf

https://jcyk.github.io/aaai2020.pdf

https://cs.emory.edu/~lzhao41/materials/papers/DynGraph2Seq\_final.pdf (Only because its Dynamic)

% Molecular
https://dl.acm.org/doi/pdf/10.1145/3340531.3411981
GitHub: https://github.com/zhichunguo/GraSeq

% AMR to text
https://github.com/freesunshine0316/neural-graph-to-seq-mp

%Link Prediction Based on Graph Neural Networks
https://proceedings.neurips.cc/paper/2018/file/53f0d7c537d99b3824f0f99d62ea2428-Paper.pdf

https://pubs.acs.org/doi/10.1021/acs.jcim.2c00321

https://github.com/freesunshine0316/neural-graph-to-seq-mp

https://arxiv.org/abs/2001.11003v2
GitHub: https://github.com/UKPLab/kg2text

Correlation metrics (Pearson, Spearman)

chrF++, METEOR, ROGUE-L

% Covers DGCNN
https://towardsdatascience.com/seal-link-prediction-explained-6237919fe575

% permutations, kendall tau
https://ecai2020.eu/papers/824\_paper.pdf

%A Data-Driven Graph Generative Model for Temporal Interaction Networks
https://dl.acm.org/doi/pdf/10.1145/3394486.3403082

https://link.springer.com/article/10.1007/s11280-020-00821-y

% Check Prediction modelling section
https://journals.plos.org/plosone/article/file?id=10.1371/journal.pone.0177630

% Jointly modeling structural and temporal self-attention
https://dl.acm.org/doi/pdf/10.1145/3336191.3371845

% Network interpolation
https://epubs.siam.org/doi/pdf/10.1137/19M1268380

https://ieeexplore.ieee.org/abstract/document/8622100

Few-shot Graph Learning for Molecular Property Prediction
https://github.com/zhichunguo/Meta-MGNN

https://dl.acm.org/doi/pdf/10.1145/3366423.3380186

% BLEU is one of the most common model-free evaluation metrics used to evaluate sequences in NLP. For BLEU score there is no brevity penalty since the length of the predicted sequence and target are always same. The BLEU-3 metric was used since for $n=3$ the sequence length is 3 and this was used for $n=4$ as well for consistency. The BLEU-3 metric considers $n$-grams up to 3. Our motivation for using this is that it would be able to capture correct pairs or triplets even if the full sequence was not correct. Also, even though 1-grams are included, they do not contribute any value since for the IOP task the predictions and target are permutations of each other. Equal weights are used for all $n$-grams.

%Since the baselines were developed only for 3-node sets in the original work, the metrics reported were accuracy and AUC. We report these metrics as a reproduction of the original work, however they are not suitable for larger node sets, we also add other metrics. For baseline evaluation we tried using BLEU-3 and Kendall's rank correlation coefficient. See appendix \ref{sec:appendix_1} for more details.

% We evaluated all experiments with $n=3$ on both datasets. 
% However, for $n=4$ the SMS-A dataset contained too few samples to be able to train a model, so we evaluated experiments with $n=4$ on only the CollegeMsg dataset.

% However, in some experiments there was no consensus as to which method was the best, for example in Table \ref{tab:seq-pred-hyperparam}. 
% Due to the discrepancy in the type of datasets used by the TAT and JODIE based models, the results were not directly comparable, so it was not possible to determine whether JODIE performed better than the baseline. 
% Metrics
